System Identification and Control of Front-Steered Ackermann Vehicles through Differentiable Physics

In this paper, we address the problem of system identification and control of a front-steered vehicle which abides by the Ackermann geometry constraints. This problem arises naturally for on-road and off-road vehicles that require reliable system identification and basic feedback controllers for various applications such as lane keeping and way-point navigation. Traditional system identification requires expensive equipment and is time consuming. In this work we explore the use of differentiable physics for system identification and controller design and make the following contributions: i)We develop a differentiable physics simulator (DPS) to provide a method for the system identification of front-steered class of vehicles whose system parameters are learned using a gradient-based method; ii) We provide results for our gradient-based method that exhibit better sample efficiency in comparison to other gradient-free methods; iii) We validate the learned system parameters by implementing a feedback controller to demonstrate stable lane keeping performance on a real front-steered vehicle, the F1TENTH; iv) Further, we provide results exhibiting comparable lane keeping behavior for system parameters learned using our gradient-based method with lane keeping behavior of the actual system parameters of the F1TENTH.

==> 2-technical_background_v0.tex <==
\section{Technical Background}\label{Technical Background}
In this section, we briefly review the theory behind the front-steered vehicle lateral \textit{error} dynamics derived in \cite{rajamani2011vehicle} and discuss the framework of DPS used for our simulations.
\subsection{Vehicle lateral Dynamics}
\begin{figure}[!htb]
\centering
\subfloat{\includegraphics[ width=4cm,height=4cm]{figures/technical_background/lane_keeping.pdf}}
\caption{A lateral lane keeping system for a front-steered vehicle.}
\label{fig:lane_keeping}
\end{figure}
 Fig. \ref{fig:lane_keeping} is a depiction of a simplified linear two-degree of freedom (2-DOF) bicycle  model of the vehicle lateral dynamics derived in \cite{rajamani2011vehicle}.
 % The original model for the vehicle lateral dynamics has sixteen state variables: twelve for the six DOF motions (three translation and three rotational) and four for the tires. A simplified linear two-degree of freedom bicycle  model of the vehicle is obtained from the complex model and as shown in Fig.\ref{fig:lane_keeping} will be used in this work. 
 2-DOF is represented by $\psi$, the vehicle yaw angle, and $y$, the lateral position with respect to the center of the rotation of the vehicle $O$.  The yaw angle is considered as the angle between horizontal \textit{vehicle body frame} axis of the vehicle, $(\Tilde{x})$, and the global horizontal axis, $(X)$. The \textit{constant} longitudinal velocity of the vehicle at its center of gravity ($\boldsymbol{CG}$) is denoted by $V_x$ and the mass of the vehicle is denoted by $m$. The distances of the front and rear tires from the $\boldsymbol{CG}$ are shown by $l_f$, $l_r$, respectively, and the front and rear tire cornering stiffness are denoted by $C_{af}$ and $C_{ar}$, respectively. The steering angle is denoted by $\delta$ which also serves as the control signal when a controller is implemented and the yaw moment of inertia of the vehicle is denoted by $I_z$. Considering the lateral position, yaw angle, and their derivatives as the state variables, and using the Newton's second law for the motion along the \textit{vehicle body frame} $\Tilde{y}-axis$, the state space model of lateral vehicle dynamics is derived in \cite{rajamani2011vehicle}. For the sake of brevity we do not discuss the state space model of the lateral vehicle dynamics here.
 
%   \begin{align} \label{eq:lat_dyn_st_sp}
%  \underbrace{\frac{d}{dt}\begin{bmatrix}
% y  \\
% \dot{y} \\
% \psi\\
% \dot{\psi} 
% \end{bmatrix}}{\dot{x}} &= 
% \begin{bmatrix}
% 0 & 1 & 0 & 0\\
% 0 & -\frac{2 C_{af}+2 C_{ar}}{m V_x} & 0 & -V_x - \frac{2 C_{af}l_f-2 C_{ar}}{m V_x} l_r\\
% 0 & 0 & 0 & 1\\
% 0 & -\frac{2 C_{af}l_f-2 C_{ar}l_r}{I_z V_x} & 0 & -\frac{2 C_{af}l_f^2+2 C_{ar}l_r^2}{I_z V_x} 
% \end{bmatrix} \nonumber\\
% &\times 
% \begin{bmatrix}
% y  \\
% \dot{y} \\
% \psi\\
% \dot{\psi} 
% \end{bmatrix} + \begin{bmatrix}
% 0  \\
% \frac{2 C_{af}}{m} \\
% 0\\
% \frac{2C_{af}l_f}{I_z}
% \end{bmatrix}\delta
% \end{align}
% Since we are primarily concerned with the lane keeping application and for the sake of brevity, we only provide the state-space representation of lateral-dynamics to a model where the state variables are the position and orientation errors with respect to the center of the lane. 
However, the error dynamics is written with two error variables : $e_1$, which is the distance between the $\boldsymbol{CG}$ of the vehicle from the center line of the lane; $e_2$, which is the orientation error of the vehicle with respect to the desired yaw angle $\psi_{des}$.
Assuming the radius of the road is $R$, the rate of change of the desired orientation of the vehicle can be defined as $\dot{\psi}_{des}= \frac{V_x}{R}$.
% \begin{align}\label{eq:des_orn}
%     \dot{\psi}_{des}= \frac{V_x}{R}
% \end{align}
The tracking or lane keeping objective of the lateral control problem is expressed as a problem  of stabilizing the following \textit{error} dynamics at the origin.
% \resizebox{.9\hsize}{!}{$A+B+C+D+E+F+G+H+I+J+K+L+M+N+O+P+Q+R+S+T+U+V+W+X+Y+Z$}
 \begin{align} \label{eq:er_dyn_st_sp}
&  \underbrace{\frac{d}{dt}\begin{bmatrix}
e_1  \\
\dot{e_1} \\
e_2\\
\dot{e_2} 
\end{bmatrix}}_{\dot{x}} =
\resizebox{0.75\hsize}{!}{  $\underbrace{\begin{bmatrix}
0 & 1 & 0 & 0\\
0 & -\frac{2 C_{af}+2 C_{ar}}{m V_x} & \frac{2 C_{af}+2 C_{ar}}{m } &  - \frac{2 C_{af}l_f-2 C_{ar}}{m V_x} l_r\\
0 & 0 & 0 & 1\\
0 & -\frac{2 C_{af}l_f-2 C_{ar}l_r}{I_z V_x} & \frac{2 C_{af}l_f-2 C_{ar}l_r}{I_z } & -\frac{2 C_{af}l_f^2+2 C_{ar}l_r^2}{I_z V_x} 
\end{bmatrix}}_{A}$} && \nonumber\\
& \times 
\underbrace{\begin{bmatrix}
e_1  \\
\dot{e_1} \\
e_2\\
\dot{e_2} 
\end{bmatrix}}_{x} + \underbrace{\begin{bmatrix}
0  \\
\frac{2 C_{af}}{m} \\
0\\
\frac{2C_{af}l_f}{I_z}
\end{bmatrix}}_{B_1}\underbrace{\delta}_{u} + \underbrace{\begin{bmatrix}
0  \\
-V_x - \frac{2 C_{af}l_f-2 C_{ar}}{m V_x} \\
0\\
-\frac{2 C_{af}l_f^2+2 C_{ar}l_r^2}{I_z V_x}
\end{bmatrix}}_{B_2} \dot{\psi}_{des}
\end{align}
 
Therefore, the above state-space form in \eqref{eq:er_dyn_st_sp} can be represented in the \textit{general} state space form as 

\begin{align} \label{eq:er_gnrl_st_sp}
\dot{x}(t) = Ax(t) + B_1(u(t)) + B_2 \dot{\Psi}_{des}
\end{align}
where $x(t)\in \mathbb{R}^n$, $t \geq 0$ is a state vector, $u(t) \in \mathbb{R}^m$, $t \geq 0$ is the control input which in this case is the steering angle $\delta$. The elements of $A \in  \mathbb{R}^{n\times n}$, $B_1, B_2 \in  \mathbb{R}^{n\times m}$ matrices are generally considered known, but in our case we obtain the elements of matrices using system identification and we assume pair $(A,B_1)$ is controllable. We also provide the definition of a closed-loop system.
\begin{definition}\label{def:closed_loop}
    The closed-loop system is defined as the system described by equation \eqref{eq:er_gnrl_st_sp}, where $u(t)=\delta_t, \forall t$, is the steering angle input to the system generated by a feedback controller .
\end{definition}




\subsection{Differentiable Physics Simulator (DPS)}
Differentiable physics simulators provide analytical gradients for physical systems, which may be used for learning-based solutions such as solving inverse problems, system identification and controller design. Enabled by the recent developments in automatic differentiation literature \cite{paszke2019pytorch, abadi2016tensorflow, al2016theano, hu2019taichi, bell2012cppad, bradbury2018jax}, a number of differentiable simulators have been proposed \cite{hu2019difftaichi, freeman2021brax, rohrbein2021differentiable, heiden2019interactive, de2018end, degrave2019differentiable, geilinger2020add, qiao2020scalable, toussaint2018differentiable, schenck2018spnets, liang2019differentiable, hu2019chainqueen}. While these simulators all aim to provide analytical gradients for learning-based methods, the variance in terms of supported features is high. In this paper, we adopt the Nimble physics simulator \cite{werling2021fast} for analytical gradient computation to develop a \textit{feedback} controller and to identify dynamic system parameters for front-steered vehicles through the control law described in Section II. Nimble physics simulator is the most suitable for our purposes because it is a  general differentiable physics simulator providing gradients through the collision mechanics between the necessary rigid body shapes for the design of a front-steered vehicle. We argue that, while it is possible to develop a differentiable simulator solely focusing on vehicle dynamics using the analytical physics equations for a vehicle model from scratch, such simulators would lack generalization capabilities and be less useful for the broader research community overall.


% a number of differentiable physics engines have been proposed to solve system identification and control problems [16, 20–22, 22, 23, 23–29]. In this work, we adopt the Nimble simulation [35] for taking advantage of the differentiation to develop control laws and identify system parameters which offers fast geometric analytical gradients through collision detection algorithms which support various types of 3D geometry and meshes. Support for various types of 3D geometry and joints is essential in order to be able to have an approximate simulation model for front-steered vehicles.


==> 3-problem_formulation_v0.tex <==
\section{Problem Formulation}\label{Problem Formulation}
At a high-level, we want to conduct simultaneous system identification and control of front-steered vehicles for a lane-keeping application. Therefore, we formulate the center lane keeping problem as a general optimization problem in terms of identified system dynamic parameters in a DPS environment as the decision variables. We use a \textit{feedback} controller of the type used in \cite{rajamani2011vehicle} as the basic controller for lane keeping with the error dynamics shown in state-space form in Eq. \eqref{eq:er_dyn_st_sp}. 

In the following sub-sections we further elaborate on our \textit{problem definition}
% In the following sub-sections we will define our problem formulation in three parts: i)the general task of lane keeping; ii) the tuning aspect of the applied \textit{feedback} controller; iii)  the learning framework for the dynamic model parameters.
\subsection{Task Representation}
Given a front steered vehicle with center of gravity $\boldsymbol{CG}$, its lateral dynamics are defined in error variables $e_1$, $e_2$ and their first-order time derivatives $\dot{e_1}$, $\dot{e_2}$, as also shown in Eq. \eqref{eq:er_dyn_st_sp}. In a simulation with total timesteps $\mathcal{T}$, the front-steered vehicle is expected to minimize the sum of the $L_2$-norms of the error dynamics states $x=\{e_1, \dot{e_1}, e_2, \dot{e_2}\}^T$ while tracking the center lane with constant longitudinal velocity $V_x$. Precisely, according to the feedback controller implementation in \cite{rajamani2011vehicle} the steady state values of $e_1$ and $e_2$ may be non-zero but should converge close to zero.
\subsection{Tuning Controller Gains}
The desired lane tracking behavior can be achieved with a feedback control structure: $\delta = -\boldsymbol{K}x = -k_1e_1 - k_2\dot{e_1} - k_3e_2 - k_4\dot{e_2}$ as also shown in \cite{rajamani2011vehicle} and the problem formulation becomes an optimization problem as follows:
\begin{equation}
\begin{aligned}\label{eq:gain_tuning}
    \min_{\boldsymbol{K}} \quad & \sum_{t=0}^{\mathcal{T}}\sqrt{e_{1,t}^2 + \dot{e}_{1,t}^2 + e_{2,t}^2 + \dot{e}_{2,t}^2}
\end{aligned}
\end{equation}
where $t$ representing the timesteps.
\subsection{Learning the Dynamic Model Parameters}
While the optimization problem defined in Eq. \eqref{eq:gain_tuning} can be solved by learning the elements of the vector $\boldsymbol{K}$ as decision variables. The open-loop matrix $A$ may have eigenvalues at the origin and be unstable. Using the state feedback law, the eigenvalues of the closed-loop matrix $(A-B\boldsymbol{K})$ can be placed at desired locations. The closed-loop system, as defined in Definition \ref{def:closed_loop}, using this state feedback controller is therefore:
\begin{equation}
\begin{aligned}\label{eq:stabilized_AB}
    \dot{x} = (A-B_1\boldsymbol{K})x + B_2 \dot{\Psi}_{des}
\end{aligned}
\end{equation}
To compute the feedback matrix $\boldsymbol{K}$, the pole placement algorithm \cite{kautsky1985robust} is used.
\begin{equation}
\begin{aligned}\label{eq:pole_placement}
    \boldsymbol{K} = place(A, B_1, P)
\end{aligned}
\end{equation}

Where the vector $P$, which is user defined, defines the desired pole locations such that the eigenvalues of the matrix $(A-B_1K)$ are negative, non-zero real numbers, satisfying the \textit{full state feedback} system stability condition. From Eq.~\eqref{eq:er_dyn_st_sp} it is observable that the matrices $A$ and $B_1$ are defined by the front-steered vehicle dynamic parameters $m$, $l_f$, $l_r$, $C_{af}$ and $C_{ar}$. Therefore, the optimization problem defined in Eq. \eqref{eq:gain_tuning} can be reformulated by replacing $\boldsymbol{K}$ with vehicle dynamic parameters as decision variables.
\begin{equation}
\begin{aligned}\label{eq:sys_id}
    \min_{{m, l_f, l_r, C_{af},  C_{ar}}} \quad & \sum_{t=0}^{\mathcal{T}}\sqrt{e_{1,t}^2 + \dot{e}_{1,t}^2 + e_{2,t}^2 + \dot{e}_{2,t}^2}
\end{aligned}
\end{equation}
% \btxt{Maybe add such that for the pole placement under the optimization formulation?}
Unlike the formulation in Eq. \eqref{eq:gain_tuning}, the optimization problem shown above with system dynamic parameters as decision variables is guaranteed to yield a stable controller structure. We hypothesize that the correct set of system dynamic parameters would yield the gain vector $\boldsymbol{K}$ that would minimize the optimization problem described in Eq. \eqref{eq:sys_id}.


==> 4-proposed_method_v0.tex <==
\section{Method}\label{Proposed Method}
In this section, we present the center lane keeping problem for front-steered vehicles as an optimization problem. To solve this problem, we also describe the design of the front-steered URDF vehicle model and the loss function formulations.
\subsection{URDF Model for Front-Steered Vehicle}
A new front-steered URDF robot model based in \cite{githubGitHubBenwarricksimple_ackermann} is designed for this line of research due to the lack of a readily available front-steered vehicle design that can be used in differentiable simulators, which are still at their early development stages and lack sophisticated simulation features like closed kinematic chain solvers. We will also share our URDF vehicle design with the general robotics community, upon successful acceptance of the script. The designed vehicle model is depicted in Fig. \ref{fig:urdf} and comprises of 7 links and 6 joints. 
% Table 1 describes the shapes and dynamic properties of these links, Table 2 describes the joint types and their properties.

\begin{figure}[!htb]
\centering
\subfloat{\includegraphics[width=7cm,height=4cm]{images/urdf-viz.pdf}}
\caption{URDF vehicle model with links' and joints' coordinate axes.}
\label{fig:urdf}
\vspace{-15pt}
\end{figure}


% \begin{table}[]
% \begin{center}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c}
% name & shape & dimensions(m) & parent joint & transformation \{xyz(m), rpy(rads)\} & mass(kg.m^2) & inertia tensor(kg)                      \\ \hline
% \multicolumn{1}{|l|}{base link} & box & [0.01 0.01 0.01] & - & - & 1 &  \multicolumn{1}{c|}{0} \\ \hline
% \multicolumn{1}{|l|}{chassis} & box & [0.8 0.2 0.01]  & base joint & \{[0 0 0], [0 0 0]\} & 5 & \multicolumn{1}{c|}{ixx=0.005, iyy=0.0187, izz=0.075} \\ \hline
% \multicolumn{1}{|l|}{right wheel} & sphere & 0.17775 & right wheel rotate & \{[0 0 0], [0 $\frac{\pi}{2}$  $\frac{\pi}{2}$]\} & 2 & \multicolumn{1}{c|}{ixx=0.041985, iyy=0.041985, izz=0.041985} \\ \hline
% \multicolumn{1}{|l|}{right wheel assembly} & sphere & 0.04 & right wheel hinge & \{[0 0 0], [0 $\frac{\pi}{2}$  $\frac{\pi}{2}$]\} & 0.2 & \multicolumn{1}{l|}{ixx=0.000128, iyy=0.000128, izz=0.000128} \\ \hline
% \multicolumn{1}{|l|}{left wheel} & sphere & 0.17775 & left wheel rotate & \{[0 0 0], [0 $\frac{\pi}{2}$  $\frac{\pi}{2}$]\} & 2 & \multicolumn{1}{c|}{ixx=0.041985, iyy=0.041985, izz=0.041985} \\ \hline
% \multicolumn{1}{|l|}{left wheel assembly} & sphere & 0.04 & left wheel hinge & \{[0 0 0], [0 $\frac{\pi}{2}$  $\frac{\pi}{2}$]\} & 0.2 & \multicolumn{1}{c|}{ixx=0.000128, iyy=0.000128, izz=0.000128} \\ \hline
% \multicolumn{1}{|l|}{right wheel rear} & sphere & 0.17775 & right wheel rear rotate & \{[0 0 0], [0 $\frac{\pi}{2}$  $\frac{\pi}{2}$]\} & 2.2 & \multicolumn{1}{c|}{ixx=0.00065, iyy=0.00065, izz=0.00065} \\ \hline
% \multicolumn{1}{|l|}{left wheel rear} & sphere & 0.17775 & left wheel rear rotate & \{[0 0 0], [0 $\frac{\pi}{2}$  $\frac{\pi}{2}$]\} & 2.2 & \multicolumn{1}{c|}{ixx=0.00065, iyy=0.00065, izz=0.00065} \\ \hline
% \end{tabular}}
% \caption{\ptxt{table captions go on the top + make table visible}Properties of the URDF robot model links}
% \label{tab:linkproperties}
% \end{center}
% \end{table}

% \begin{table}[]
% \begin{center}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c|c}
%   name & type & parent link & child link & translation (xyz)(m) & axis(xyz)                      \\ \hline
% \multicolumn{1}{|l|}{base joint} & fixed & base link & chassis & - & \multicolumn{1}{c|}{-} \\ \hline
% \multicolumn{1}{|l|}{right wheel hinge} & revolute & chassis & right wheel assembly & [0.4 0.125 0] & \multicolumn{1}{c|}{[0 0 1]} \\ \hline
% \multicolumn{1}{|l|}{right wheel rotate} & continuous & right wheel assembly & right wheel & [0 0.025 0] & \multicolumn{1}{c|}{[0 1 0]} \\ \hline
% \multicolumn{1}{|l|}{left wheel hinge} & revolute & chassis & left wheel assembly & [0.4 -0.125 0] & \multicolumn{1}{c|}{[0 0 1]} \\ \hline
% \multicolumn{1}{|l|}{left wheel rotate} & continuous & left wheel assembly & left wheel & [0 -0.025 0] & \multicolumn{1}{c|}{[0 1 0]} \\ \hline
% \multicolumn{1}{|l|}{right wheel rear rotate} & continuous & chassis & right wheel rear & [-0.4 0.15 0] & \multicolumn{1}{c|}{[0 1 0]} \\ \hline
% \multicolumn{1}{|l|}{left wheel rear rotate} & continuous & chassis & left wheel rear & [-0.4 -0.15 0] & \multicolumn{1}{c|}{[0 1 0]} \\ \hline
% \end{tabular}}
% \caption{Properties of the URDF robot model joints}
% \label{tab:jointproperties}
% \end{center}
% \end{table}

\subsection{Vehicle Initialization and Trajectory Design}\label{sec:Vehicle Initialization and Trajectory Design}
% \btxt{Initialization and setup conditions given here can also be given in simulation set-up. Alternatively, I can give general forms and give values for each parameters in simulation set-up.}
The vehicle is initialized in simulation experiments at the origin of the 2-Dimensional (2D) Cartesian coordinate frame with zero radians of heading offset with respect to the $\hat{y}$-axis. Center-lane trajectories are defined as circular trajectories with a center offset.
\begin{equation}
\begin{aligned}\label{eq:circle_eqn}
    (\hat{x}-h)^2 + (\hat{y}-k)^2 = r^2
\end{aligned}
\end{equation}
where the $\hat{y}$-axis offset $k$ is fixed to $1\ m$ and the $\hat{x}$-axis offset is equal to the uniform randomly sampled radius in arbitrary direction along the $\hat{x}$-axis: $h=\pm r$. Note that for the DPS simulator we define the \textit{global } frame axes as $\hat{x}$ and $\hat{y}$.

\subsection{Loss Function}
The loss function needs to enforce the vehicle to follow the center lane trajectory and is defined as follows:
\begin{equation}
\begin{aligned}\label{eq:Lcl}
    \mathcal{L}_{cl} = \sum_{t=t_{cls}}^{\mathcal{T}}\sqrt{e_{1,t}^2 + \dot{e}_{1,t}^2 + e_{2,t}^2 + \dot{e}_{2,t}^2}
\end{aligned}
\end{equation}

\noindent where $t_{cls}$ defines the starting timestep for the center lane keeping loss. Due to the vehicle inertia, before the vehicle reaches the desired velocity $V_x$, the loss term gets  biased towards the loss terms in the beginning of the simulation timesteps. Therefore a time offset is necessary to mitigate this bias. Note that the loss $\mathcal{L}_{cl}$ does not penalize the simulated vehicle for not moving at all. Therefore another loss term for the longitidunal velocity is defined:

\begin{equation}
\begin{aligned}\label{eq:Lvel}
    \mathcal{L}_{vel} =\frac{1}{\mathcal{T}-t_{vs}} \sum_{t=t_{vs}}^{\mathcal{T}}|V_x - \widetilde{V_x}|
\end{aligned}
\end{equation}

\noindent where $t_{vs}$ defines the starting timestep for the velocity loss and $\widetilde{V_x}$ defines the actual longitudinal velocity of the vehicle. Since the vehicle is initialized with zero velocity, due to inertia, the simulated vehicle requires a time offset to reach the required $V_x$. A weighted linear combination of $\mathcal{L}_{vel}$ and $\mathcal{L}_{cl}$ is proposed as the actual loss function:

\begin{equation}
\begin{aligned}\label{eq:Ltot}
    \mathcal{L} = \mathcal{L}_{cl} + \lambda\mathcal{L}_{vel}
\end{aligned}
\end{equation}
Where the weight is empirically determined as $\lambda = 5000$. In practice, the sudden changes in derivative error variables $\dot{e_1}$ and $\dot{e_2}$ destabilize the steering behavior. Therefore, derivative error variables are smoothed using an exponential moving average:
\begin{equation}
\begin{aligned}\label{eq:ema}
    \dot{e}_{1,t} = (1-\alpha)\dot{e}_{1,t-1} + \alpha(e_{1,t}-e_{1,t-1}) \\
    \dot{e}_{2,t} = (1-\alpha)\dot{e}_{2,t-1} + \alpha(e_{2,t}-e_{2,t-1})
\end{aligned}
\end{equation}
Where the smoothing coefficient $\alpha$ is empirically set to $10^{-3}$.

\subsection{Differentiable Physics}
The pseudo code for differentiable forward physics computation is shown in Algorithm \ref{algo:pseudocode-1} and its structure is also depicted in Fig.\ref{fig:dps_framework}. An epoch of forward physics simulation takes the system parameters $\hat{P}=[m, l_f, l_r, C_{af}, C_{ar}]^T \in \mathbb{R}^{5}$ and a reference trajectory, denoted by $\hat{r}$, as input and computes the loss $\mathcal{L}$ for accumulating the error variables. Line 1 initializes the loss and the error variables at simulation start. In line 2, $\tilde{\omega}$ is the desired angular velocity for the rear wheels and $r_{w}$ is the vehicle's wheel radii. In Line 3, the A and $B_{1}$ matrices are computed for the state-space dynamics. In line 4, we use our own differentiable implementation of the pole placement algorithm based on SciPy \cite{virtanen2020scipy} implementation of the KNV \cite{kautsky1985robust} pole placement algorithm. Enabled by PyTorch automatic differentiation capabilities, our differentiable implementation of the $place$ function allows us to backpropagate the gradients to the system parameters through the A and $B_1$ matrices, which lets us identify the dynamic system parameters. Line 5 describes the iterative process over the DPS timesteps. In line 6, our feedback controller computes the steering angle $\delta_{t}$. Line 7 describes the DPS state, $s_{t+1}$ , propagation step, which takes in the current state and our inputs and generates the next state. Note that the DPS states denoted by $s_t$ represent the full environment state for every object, that is full pose: $3$-position $\hat{x},\hat{y},\hat{z}$ and $3$-rotation in axis-angle.  In line 8, we compute the error variables $x_{t+1}$ and our vehicle's longitudinal velocity $\tilde{V}_{x,t+1}$. In lines 9-10 we accumulate the losses defined in Eq. \eqref{eq:Lcl},\eqref{eq:Lvel} and \eqref{eq:Ltot}.

\subsubsection*{Backward Computation} Since the differentiable physics simulations provide us with the analytical gradients, the gradients of the loss function with respect to the system parameters described by the following equation are provided to us by the simulator for gradient-based optimization:

% \begin{equation}
% \begin{aligned}\label{eq:backward_eqn}
%     \frac{\partial\mathcal{L}}{\partial p_{i}} = \frac{\partial\mathcal{L}_{cl}}{\partial p_{i}} + \lambda \frac{\partial\mathcal{L}_{vel}}{\partial p_{i}}
% \end{aligned}
% \end{equation}
\begin{equation}
\begin{aligned}\label{eq:backward_eqn}
    \frac{\partial\mathcal{L}}{\partial p_{i}} = \sum_{j=1}^4 \left(\frac{\partial\mathcal{L}_{cl}}{\partial K_{j}}\cdot \frac{\partial K_{j}}{\partial p_{i}} + \lambda \Big (\frac{\partial\mathcal{L}_{vel}}{\partial K_{j}} \cdot \frac{\partial K_{j}}{\partial p_{i}}\Big )\right )
\end{aligned}
\end{equation}

\noindent where $p_{i} \in \hat{P}$ is the $i^{th}$ dynamic system parameter and $K_j$ is the $j^{th}$ gain element in $\boldsymbol{K}\in \mathbb{R}^4$.
% Clearly, in Eq. \eqref{eq:backward_eqn}, the derivative of the \textit{total} loss function $\mathcal{L}$ with respect to the system parameters is a function of the derivative of the individual loss functions $\mathcal{L}_{cl}$ and $\mathcal{L}_{vel}$ with respect to the gains and the derivative of the gains with respect to the system parameters. 
Eq. \eqref{eq:backward_eqn} implies that minimizing the loss functions tunes the gains for reducing the lateral error with respect to the lane centerline and velocity tracking error with respect to $V_x$, the reference velocity. In turn, the gains are a direct function of the system parameters $\hat{P}$ as the gains are derived from the \textit{pole placement} method given by Eq. \eqref{eq:pole_placement}. This is also why we take the derivative of the total loss function $\mathcal{L}$ with respect to the system parameters in the first place.



\begin{algorithm}
\caption{Forward Computation ($\hat{P}$, $\hat{r}$)}\label{algo:pseudocode-1}
\begin{algorithmic}[1]
\State $\mathcal{L} = 0$, $x_0=\{e_{1,0}, \dot{e}_{1,0}, e_{2,0}, \dot{e}_{2,0}\}^T$
\State $\tilde{\omega}$ = $\frac{V_x}{r_{w}}$

\State $A, B_{1}=AB\_matrix(\hat{P})$ 
\State $\boldsymbol{K}=place(A,B1)$
\For{\texttt{t = 0...$\mathcal{T}$}}
    \State $\delta_{t}$ = $-\boldsymbol{K}x_t$
    \State $s_{t+1}$ = $DPS(s_t,\tilde{\omega},\delta_{t})$
    \State $x_{t+1}, \tilde{V}_{x,t+1}$ = $compute\_errors(s_{t+1}, \hat{r})$
    \State $\mathcal{L}_{cl,t}=x_{t+1}$, $\mathcal{L}_{vel,t}=|V_{x}-\tilde{V}_{x,t+1}|$
    \State $\mathcal{L}\mathrel{+}=$ 
    $\mathcal{L}_{cl,t} + \mathcal{L}_{vel,t}$    
\EndFor

\State \Return $\mathcal{L}$

\end{algorithmic}
\end{algorithm}


==> 5-simulation_results_v0.tex <==
\section{Simulation Results}\label{Simulation Results}
The front-steered vehicle was run for $\mathcal{T} = 7000$ timesteps in Nimble \cite{werling2021fast} differentiable physics simulator with each timestep corresponding to 0.001 seconds. Time offsets are empirically set as $t_{cls}=2000$ and  $t_{vs}=2500$. For training epochs, batch size is set to 2 for AdamW optimizer \cite{loshchilov2018decoupled} and circular trajectory radii was uniformly sampled from the interval $[25m,35m]$ and centered with the offsets defined in Section \ref{sec:Vehicle Initialization and Trajectory Design}. A single validation epoch is run every $4$ training epochs with circles placed on the positive and negative side of the $\hat{x}$-axis, with radii $\{25m,35m\}$. Training is stopped if the loss does not improve for $5$ validation epochs for the gradient-based optimization. Loss and parameter figures are plotted as the average of $5$ separate training rounds with uniformly sampled initial parameters. Since we use the early stopping technique for gradient-based optimization, the lines describing gradient-based training may terminate early before they reach the full number of epochs. Additionally, if there are less than $2$ loss or parameter (y-value) values remaining at a training epoch for gradient-based optimization, we also omit the remaining part for plotting purposes. For all rounds of all experiments, the coefficient of friction between the vehicle wheels and the ground was set to $\mu=1.0$ and the steering angles were clipped at each timestep, to be in the interval: $[-\frac{\pi}{4}, \frac{\pi}{4}]$. Additionally, the front and rear wheel cornering stiffness values $C_{af}$ and $C_{ar}$ were constrained to be equal during the optimization as well as the front and rear wheels' longitudinal distances $\l_{f}$,$\l_{r}$, from the center of gravity of the vehicle. The feedback controller poles were set as $P=[-5,-4,-7,-10]$ since negative pole placement is necessary for the stability of the controller. As baselines, gradient-free optimizers TPE \cite{bergstra2011algorithms} and CMA-ES \cite{hansen2016cma} are used for single and multi parameter optimizations, respectively, from the Optuna library \cite{akiba2019optuna}. An important detail to be mentioned is that the gradient-free baselines can propose values for $\boldsymbol{K}$ gains or system dynamic parameters that can yield an unstable controller with NaN loss value, these NaN values are ignored during the averaging.
\vspace{-2.5pt}
% \btxt{Maybe rewrite the problem as a constrained optimization problem as equation?}

\subsection{Model Identification}
In this section, we present the gradient-based optimization of the gain parameters and compare it to the gradient-free baseline.
For gradient-based optimization of the gain parameters, the elements of $\boldsymbol{K}$ are initialized at zero. The learning rate for the optimizer is set to $0.2$ and gradient clipping threshold is set to $1000$ for the $L_2$-norm of the gradient of the loss term with respect to $\boldsymbol{K}$. At every epoch, the gradient-free baseline is constrained to suggest a floating-point number for each of the elements of $\boldsymbol{K}$ from the interval: $[-2.5,2.5]$. Since we don't have any condition enforcing the stability of the vehicle, the training epochs may return NaN values. We present the loss curves for gradient-based and gradient-free gain optimizations in Fig. \ref{fig:K_optim_results} for 64 epochs. Compared to gradient-free baseline, our gradient-based method provides higher sample-efficiency and a more regular loss curve enabled by the analytical gradients. The effect of the analytical gradients is particularly evident in the first few epochs where gradient-based methods have to initially explore the search space.



\begin{figure}[!htb]
\vspace{-10pt}
\centering
% \subfloat[Kdiff]
{\includegraphics[width = 0.8\linewidth]{figures/gain_tuning/K.pdf}}
\caption{Plot shows the loss trend for the optimization of the feedback gains $\boldsymbol{K}$. Since the direct optimization of gains does not have any constraints for stability, the gradient-free CMA-ES baseline can propose infeasible gains which may output NaN values for the errors as observed near 10 epochs.}
\vspace{-10pt}
\label{fig:K_optim_results}
\end{figure}


%\subsection{Analytical Dynamic Model Parameter Learning}\label{sec:adm}
As discussed in Section \ref{Problem Formulation}, optimized $\boldsymbol{K}$ gains do not necessarily yield a stable controller structure. By backpropagating the gradients to the system dynamic parameters assumed by the control law, we iteratively improve the center lane tracking performance while keeping the stability conditions proposed by the pole placement feedback controller. The URDF model explicitly defines the system dynamic parameters as $m=14.8\ kg$, $\l_f = \l_r = 0.4\ m$. Applying the parallel axis theorem \cite{haas1925introduction}, the vehicle yaw moment of inertia $I_z$ is computed as $1.764\ kg.m^2$. In this sub-section, we first run the gradient-based optimization process with the tire cornering stiffness $C_{af}$ parameter as the decision variable (Fig. \ref{fig:Caf-param-optim-results}) due to the $C_{af}=C_{ar}$ constraint. At the beginning of each training round $C_{af}$ parameter is initialized by uniform sampling from the interval: $[10.0 ,50.0] \ N/rad$ . Then the $C_{af}$ and $C_{ar}$ parameters are assumed to be known and the optimization is ran with the vehicle mass $m$ as the decision variable in Fig.~\ref{fig:m-param-optim-results}. The initialization range for the $m$ is $[0.5,40]\ kg$. The third optimization task uses vehicle mass and cornering stiffness parameters jointly as independent decision variables in Fig.~\ref{fig:caf-m-param-Caf-results} and Fig.~\ref{fig:caf-m-param-m-results}. The optimizer learning rates for both $m$ and $C_{af}$ parameters were set to 1.0. The gradient clipping $L_2$-norm thresholds for $m$ and $C_{af}$ were set to 100 and 10, respectively.

\subsubsection*{\textbf{Learning the Tire Cornering Stiffness Parameter}} In Fig.~\ref{fig:Caf-param-optim-results}, we present the value of the $C_{af}$ parameter used by the feedback controller over training epochs with the rest of the dynamic system parameters used by the controller set to their actual physical values as discussed in Section~\ref{sec:adm}. Our experiments validate that our gradient-based method converges to $13.5\ N/rad$ in fewer samples compared to the gradient-free baseline. 

% \subfloat[gb-Caf-param]{\includegraphics[width = 0.9\linewidth]

\begin{figure}
\centering
% \subfloat[gb-Caf-param]
{\includegraphics[width = 0.8\linewidth]{figures/single-parameter/Caf/Caf-param.pdf}}

\caption{Plot shows the learning trend for the cornering stiffness parameter of the controller over the epochs. The black line represents the final converged value for the cornering stiffness. Our gradient-based optimizer stops training if the loss does not decrease for 6 validation epochs.}
\vspace{-10pt}
\label{fig:Caf-param-optim-results}
\end{figure}
\subsubsection*{\textbf{Learning the Mass Parameter}} Similar to the previous sub-section, we set the rest of the dynamic system parameters used by the controller to their physical values except for $m$ and $C_{af}$, where $C_{af}$ is set to $13.5\ N/rad$ as identified in the previous sub-section. We run our gradient-based method and gradient-free baseline for the identification of $m$. For the mass, both of the optimizers show comparable performance as depicted in Fig. \ref{fig:m-param-optim-results}, which indicates that for single dimensional search spaces the sample efficiency provided by having the analytical gradients not necessarily be as useful as it was hypothesized initially.
\begin{figure}
\centering
% \subfloat[gm-param]
{\includegraphics[width = 0.8\linewidth]{figures/single-parameter/m/m-param.pdf}}
\caption{Plot shows the learning trend for the mass parameter of the controller over the epochs. The black line represents true mass of the vehicle. Our gradient-based optimizer stops training if the loss does not decrease for 6 validation epochs.}
\vspace{-10pt}
\label{fig:m-param-optim-results}
\end{figure}


\subsubsection*{\textbf{Jointly Learning the Mass and the Tire Cornering Stiffness}} Finally we run our gradient-based method by setting the dynamic system parameters $m$ and $C_{af}$ used by the controller as decision variables and the rest of the parameters to their physical values as defined by the URDF model. Fig.~\ref{fig:caf-m-param-Caf-results} and Fig.~\ref{fig:caf-m-param-m-results} show the convergence of the learnable parameters over training epochs. In Fig. \ref{fig:caf-m-param-Caf-results}, both of the optimizers converge to a larger than expected value for $C_{af}$ while in Fig. \ref{fig:caf-m-param-m-results}, for the mass, the gradient-based method converges to the ground truth while the gradient-free baseline converges to a significantly larger value. Although the identified system parameter values are not very accurate, the controller performance is still good
% The conclusion we draw from this result is that good controller performance does not necessarily correspond with an accurate system parameter identification and controller error can only serve as an approximate proxy for system identification. 
 as corroborated by the error profile in Fig.~\ref{fig:caf-m-param-m-results}
 % , we present the error profile of the controller 
 for the jointly gradient-based identified system parameters $m=14.35\ kg$ and~$C_{af}=15.37\ N/rad$.
 % with rest of the dynamic system parameters set to their physical values as presented in Section \ref{sec:adm}.

%\begin{figure}
%\centering
%\subfloat[]{\includegraphics[width=9cm,height=5cm]{figures/multi-parameter/Caf-m/Caf-joint.pdf}}\label{fig:caf-m-param-Caf-results}
%\subfloat[]{\includegraphics[width=4cm,height=2cm]{figures/multi-parameter/Caf-m/m-joint.pdf}}\label{fig:caf-m-param-m-results}
%\caption{}
%\end{figure}


\begin{figure}
\centering
 %\subfloat[gb-Caf-m-param-Caf]
{\includegraphics[width = 0.8\linewidth]{figures/multi-parameter/Caf-m/Caf-joint.pdf}}
\caption{Plot shows the learning trend for the cornering stiffness parameter of the controller over the epochs of the cornering stiffness and mass parameters' joint learning. The black horizontal line represents the identified cornering stiffness value through gradient-based learning in Fig. \ref{fig:m-param-optim-results}. Our gradient-based optimizer stops training if the loss does not decrease for 6 validation epochs.}
\label{fig:caf-m-param-Caf-results}
\end{figure}
\begin{figure}
\centering
% \subfloat[gb-Caf-m-param-m]
{\includegraphics[width = 0.8\linewidth]{figures/multi-parameter/Caf-m/m-joint.pdf}}
\caption{Plot shows the learning trend for the mass parameter of the controller over the epochs of the cornering stiffness and mass parameters' joint learning. The black horizontal line represents the true mass of the vehicle. Our gradient-based optimizer stops training if the loss does not decrease for 6 validation epochs.}
\label{fig:caf-m-param-m-results}
\end{figure}

\begin{figure}
\centering
\subfloat[]{\includegraphics[width = 0.5\linewidth]{figures/pybullet/bullet_ep.pdf}\label{fig:bullet-errors}}
\subfloat[]{\includegraphics[width = 0.5\linewidth]{figures/multi-parameter/Caf-m/joint_profiled_errors.pdf}\label{fig:Caf_m_error_profile}}

% \subfloat[]{\includegraphics[width = 0.5\linewidth]{sim_images/MULTIWEED_turnRweedsDetected.eps}}\\
\caption{The plots show trends over 7000 simulation timesteps (7s) in $e_1$ and $e_2$ (a) PyBullet (b) Nimble physics for controller based on identified system parameters on separate trajectories.}
\vspace{-10pt}
\end{figure}

==> 6-generalization_experiments_v0.tex <==
\section{Generalization Experiment Results}\label{Generalization Experiment Results}

To test the generalizability of our method and environment models, we also evaluated the optimized controller in PyBullet \cite{coumans2021}, which is a widely used physics simulator in literature and is not natively differentiable. Using the same URDF models for the ground plane and the front-steered vehicle, with the controller gains set as $\boldsymbol{K}=[46.92, 11.00, 2.74, -1.06]$ through the joint identification of system parameters as presented in Section~\ref{sec:adm}. The error profiles presented in Fig. \ref{fig:bullet-errors} for $e_1$ and $e_2$ demonstrate that model designs are transferable across simulators and optimized controllers show similar performance. 
% It should also be noted that the error profiles generated from Nimble physics simulator and PyBullet have slight differences in terms of simulation timesteps elapsed before the controller becomes active (observable as slight shift in trend around $1000^{th}$ timestep in Fig. \ref{fig:bullet-errors}). This is the result of slight differences between different simulators at handling velocity controls and frictional forces.
Video submitted with this paper provides extensive results from simulations conducted on both Nimble physics and PyBullet simulators. 
% width = 0.8\linewidth
% width=9cm,height=5cm

